Plasticity of the unit ball of $c$ and $c_0$

We prove the plasticity of the unit ball of $c$. That is, we show that every non-expansive bijection from the unit ball of $c$ onto itself is an isometry. We also demonstrate a slightly weaker property for the unit ball of $c_0$ -- we prove that a non-expansive bijection is an isometry, provided that it has a continuous inverse.

==> c0_proofs/c0_step4_v1.tex <==
\begin{lemma}\label{c0_step4}
    Let $y\in B_0$ and $n\in\N$. If $y_n=0$ and $y_i\ne 0$ for all $i\ne n$, then $\tildeF^{-1}(y)_n=0$.
\end{lemma}
\begin{proof}
    Construct sequences $z\in B_0$ and $w\in B_0$ as follows:
    \begin{itemize}
        \item let $z_n=1$, let $w_n=-1$;
        \item for $i\ne n$, let $z_i=w_i=y_i$.
    \end{itemize}
    Denote elements $\tildeF^{-1}(y)$, $\tildeF^{-1}(z)$ and $\tildeF^{-1}(w)$ by $y'$, $z'$ and $w'$. Note that the distance between $y$ and $z$ is equal to one and the distance between $y$ and $w$ is also equal to one. Therefore, the distance between $y'$ and $z'$ is at least one and the distance between $y'$ and $w'$ is also at least one.
    
    Lemma \ref{c0_step3a} implies that $z'_n=1$ and $w'_n=-1$. Consider an index $i\ne n$. We know that $y_i\ne 0$, so either $y_i<0$ or $y_i>0$. If $y_i<0$, then Lemma \ref{c0_step3a} implies that $y'_i$, $z'_i$ and $w'_i$ are all negative, which means that $|y'_i-z'_i|<1$ and $|y'_i-w'_i|<1$. Similarly, if $y_i>0$, then $y'_i$, $z'_i$ and $w'_i$ are all positive, thus $|y'_i-z'_i|<1$ and $|y'_i-w'_i|<1$.
    
    Consider the elements $y'$ and $z'$. We know that we have $|y'_i-z'_i|<1$ for all $i\ne n$. Let us show that $|y'_n-z'_n|\geq 1$. Suppose by contrary that $|y'_n-z'_n|<1$. Then we have $|y'_i-z'_i|<1$ for every $i\in\N$. It follows that $\|y'-z'\|<1$, because every element of $c_0$ should attain its norm. This is a contradiction, because we know that the distance between $y'$ and $z'$ should be at least one. Therefore, we must have $|y'_n-z'_n|\geq 1$. The last fact implies that $y'_n\leq 0$. Now we can repeat the above argument for $y'$ and $w'$ to obtain the inequality $y'_n\geq 0$. Combining these two together, we get $y'_n=0$.
\end{proof}
